Multitask Learning Can Improve Worst-Group Outcomes

In order to create machine learning systems that serve a variety of users well, it is vital to not only achieve high average performance but also ensure equitable outcomes across diverse groups. However, most machine learning methods are designed to improve a model's average performance on a chosen end task without consideration for their impact on worst group error. Multitask learning (MTL) is one such widely used technique. In this paper, we seek not only to understand the impact of MTL on worst-group accuracy but also to explore its potential as a tool to address the challenge of group-wise fairness. We primarily consider the standard setting of fine-tuning a pre-trained model, where, following recent work \citep{gururangan2020don, dery2023aang}, we multitask the end task with the pre-training objective constructed from the end task data itself. In settings with few or no group annotations, we find that multitasking often, but not consistently, achieves better worst-group accuracy than Just-Train-Twice (JTT; \citet{pmlr-v139-liu21f}) -- a representative distributionally robust optimization (DRO) method. Leveraging insights from synthetic data experiments, we propose to modify standard MTL by regularizing the joint multitask representation space. We run a large number of fine-tuning experiments across computer vision and natural language processing datasets and find that our regularized MTL approach \emph{consistently} outperforms JTT on both average and worst-group outcomes. Our official code can be found here: \href{https://github.com/atharvajk98/MTL-group-robustness.git}{\url{https://github.com/atharvajk98/MTL-group-robustness}}.

==> sections/avg_acc_discussion.tex <==
\subsection{Impact on Average Accuracy under different settings}
\label{sec:results_avg}

\subsubsection{Multitasking improves average performance}
% \ak{Editing in progress} \\
\begin{wrapfigure}[20]{r}{0.57\textwidth}
\vspace{-3mm}
  \begin{center}
    \includegraphics[width=0.57\textwidth]{images/box_plot_aga.pdf}
  \end{center}
  % \vspace{-3mm}
  \caption{\label{fig:result_avg} Regularized MTL improves average group accuracy when group annotations are available}
\end{wrapfigure}
% \begin{figure*}[!htb]
%     \centering
%     \includegraphics[scale=0.2]{images/average_acc_box_whister_plot.pdf}
%     \caption{Regularized MTL improves average group accuracy when group annotations are available}
%     \label{fig:result_avg}
% \end{figure*}
Figure \ref{fig:result_avg} illustrates the performance of ERM, JTT, and our approach concerning average accuracy. Constrained multitasking with the pre-training objective consistently improves performance across both datasets when validation group annotations are available. Therefore, when considering both Figure \ref{fig:no_group_data} and \ref{fig:result_avg}, it becomes evident that our method not only yields superior average performance but also excels in worst-case scenarios. In cases where group annotations are absent, our method achieves slightly lower results, though still exceeding $97\%$. However, juxtaposing the results in Figure \ref{fig:no_group_data} and \ref{fig:result_avg}, we see that our approach achieves a better trade-off between average and worst-case accuracy across both datasets. Thus, our empirical findings align with our theoretical investigation, demonstrating that our method effectively reduces spurious features in shared representations and enhances generalization across all sub-groups.

\subsubsection{Are both regularization and multitasking jointly necessary?}
\label{sec:results_avg}
% \ak{Editing in progress} \\
\begin{table}[h!]
    % \caption{Regularization ablations}
    % \vspace{-3mm}
    \begin{minipage}{.5\linewidth}
      \centering
      \caption{\label{tab:reg_ablate_wb_avg} Waterbirds Ablation}
      % \vspace{-3mm}
        \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \multicolumn{2}{c}{\textbf{Group Labels}}  \\ 
        & None & Validation \\ \midrule
ERM &  $95.5_{0.2}$  & $94.1_{0.7}$ \\ 
\quad + L1 &  $95.6_{0.3}$ & $94.7_{0.9}$ \\ 
\quad + MIM & $95.3_{0.4}$  & $95.0_{0.6}$ \\ 
\quad + MIM + L1 & $\boldsymbol{95.8}_{0.3}$ & $\boldsymbol{95.4}_{0.4}$ \\
\bottomrule
        \end{tabular}%
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
      \caption{\label{tab:reg_ablate_cvs_avg} Civilcomments-small Ablation}
      % \vspace{-3mm}
        \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \multicolumn{2}{c}{\textbf{Group Labels}}  \\ 
        & None & Validation \\ \midrule
        ERM &  $83.9_{0.4}$ &  $81.4_{1.0}$ \\ 
        \quad + L1 &  $83.7_{0.4}$ & $80.3_{0.7}$ \\
        \quad + MLM &  $83.9_{1.2}$ & $81.1_{1.1}$ \\
        \quad + MLM + L1 & $\boldsymbol{84.4}_{0.4}$ & $\boldsymbol{82.0}_{0.5}$ \\
        \bottomrule
        \end{tabular}%
    \end{minipage} 
    % \vspace{-3mm}
\end{table}

Tables \ref{tab:reg_ablate_wb_avg} and \ref{tab:reg_ablate_cvs_avg} present ablation studies focusing on average accuracy. Consistent with the findings in Section \ref{sec:results_avg}, we observe that incorporating L1 regularization into multitask learning with the pre-trained objective produces the highest average accuracy when validation annotations are accessible. In line with the theoretical findings, the synergy between L1 regularization and MLM/MIM results in stable trade-offs between average and worst-group accuracy.


\subsubsection{Going beyond the pre-training objective}
% \ak{Editing in progress} \\
\begin{table}[h!]
    % \vspace{-3mm}
    % \caption{\label{tab:obj_ablate_wb} Ablating the choice of auxiliary task}
    % \vspace{-1mm}
    \begin{minipage}{.5\linewidth}
      \centering
      \caption{\label{tab:obj_ablate_wb_avg} Waterbirds: MIM $\rightarrow$ SimCLR}
      % \vspace{-3mm}
        \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \multicolumn{2}{c}{\textbf{Group Labels}}  \\ 
        & None & Validation \\ \midrule
ERM &  $95.5_{0.2}$  & $94.1_{0.7}$ \\ 
\quad + MIM + L1 & $95.8_{0.3}$ & $95.4_{0.4}$ \\
\quad + SimCLR + L1 & $\boldsymbol{96.1}_{0.3}$ & $\boldsymbol{95.5}_{0.7}$ \\
\bottomrule
        \end{tabular}%
    \end{minipage}%
% \vspace{-3mm}
    \begin{minipage}{.5\linewidth}
      \centering
      \caption{\label{tab:obj_ablate_cvs_avg} Civilcomments-small: MLM $\rightarrow$ CLM}
      % \vspace{-3mm}
        \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \multicolumn{2}{c}{\textbf{Group Labels}}  \\ 
        & None & Validation \\ \midrule
        ERM &  $83.9_{0.4}$ &  $81.3_{0.9}$ \\ 
        \quad + MLM + L1 & $\boldsymbol{84.4}_{0.4}$ & $\boldsymbol{82.0}_{0.5}$ \\
\quad + CLM + L1 &  $83.3_{0.7}$ & $81.1_{0.9}$ \\ 
        \bottomrule
        \end{tabular}%
    \end{minipage} 
    % \vspace{-1mm}
\end{table}

The results presented in Tables \ref{tab:obj_ablate_wb_avg} and \ref{tab:obj_ablate_cvs_avg} elucidate the impact of multitasking using various transfer learning objectives on average accuracy. In line with the observations in Section \ref{ref:beyond_core_obj}, SimCLR consistently delivers results that are either superior or comparable to those achieved with the masked image modeling objective. Interestingly, CLM outperforms MLM when assessed based on average validation accuracy checkpointing. However, a comparison with Table \ref{obj_ablate_cvs} reveals a significant disparity between the average and worst-group performance in the case of CLM.


==> sections/loss_weight_effect.tex <==
% \subsection{Impact of $\boldsymbol{w_{\mathrm{ssl}}}$ and $\boldsymbol{w_{\mathrm{reg}}}$}
\subsection{Impact of Loss Weighing}
\label{sec:loss_weighting}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{images/L1_effect_mean_acc.pdf}
    \caption{Effect of L1 regularization weight on the trade-off between average and worst-group performance.}
    \label{fig:L1_effect_mean_acc}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.9\textwidth]{images/MT_effect_mean_acc.pdf}
    \caption{Effect of self-supervised (ssl) auxiliary objective weight on the trade-off between average and worst-group performance.}
    \label{fig:MT_effect_mean_acc}
\end{figure*}

Figures \ref{fig:L1_effect_mean_acc} and \ref{fig:MT_effect_mean_acc} depict the influence of $w_{\mathrm{ssl}}$ and $w_{\mathrm{reg}}$ on the trade-off between average and worst group accuracy. Every point depicted on the Pareto front is represented by the mean average accuracy (x-axis) and mean worst-group accuracy (y-axis) across different hyperparameter configurations. In both the Waterbirds and Civilcomments-small datasets, we consistently observe that setting $w_{\mathrm{reg}}$ to $e^{-1}$ results in the best performance. This configuration consistently outperforms $w_{\mathrm{reg}} = 1$ and $w_{\mathrm{reg}} = 0$, highlighting the importance of L1 regularization in enhancing both average and worst-group performance, albeit with a smaller weight coefficient. Notably, when $w_{\mathrm{reg}}$ exceeds 1, there is a significant drop in performance, indicating a substantial reduction in the representation capacity of the shared representation layer. In summary, the Pareto front captures the importance of L1 regularization for achieving performance gains across average and worst-group performance. The influence of $w_{\mathrm{ssl}}$ varies between the datasets, and it is challenging to precisely quantify the effect of different $w_{\mathrm{ssl}}$ values.



==> sections/theory_extended.tex <==
\section{Theory Details}
\subsection{Definitions, Setup and Pre-Work}
We consider the case where the main task and the transfer task are both binary classification tasks over the same input space. Specifically, we have the input space $\mathcal{X} = \mathbb{R}^{d}$ and the output space $\mathcal{Y} = \{-1, 1\}$. We repeat the setup from Section \ref{sec_theory} here for ease of access.
\subsection{End-Task}
The primary task is defined by $\mathbf{T}_{\mathrm{prim}} = \{(x_i, y_i)\}_{i \in N}$ where we have $N$ total samples. A spurious attribute $a \in \{-1, 1\}$ divides the training set samples into four groups. The data is dominated by samples where $\{a = y\}$ and thus we have two majority groups $\mathbf{G}_{a = y = 1}, \mathbf{G}_{a = y = -1}$ each with $\frac{n_{\mathrm{maj}}}{2}$ samples. The two minority groups are when $\{a = -y\}$ each with $\frac{n_{\mathrm{min}}}{2}$ : $\mathbf{G}_{a = -y = 1}, \mathbf{G}_{a = -y = -1}$ . Due to the fact that  $n_{\mathrm{maj}} > n_{\mathrm{min}}$, the attribute $a$ is highly correlated with the label $y$ in the training data and is thus a spurious feature when considering the generative distribution : 
\begin{equation}
\label{eqn:prim_gen_dist}
    \begin{split}
        x_{\mathrm{core}} ~|~ y &~ \sim \mathcal{N}\left(y\mathbf{1} ~,~ \sigma^2_{\mathrm{core}}I_{d_c} \right) \\
        x_{\mathrm{spur}} ~|~ a &~\sim \mathcal{N}\left(a\mathbf{1} ~,~ \sigma^2_{\mathrm{spur}}I_{d_s} \right) \\
    \end{split} 
\end{equation}
$$x = [x_{\mathrm{core}}; x_{\mathrm{spur}}] \in \mathbb{R}^d \quad \text{and} \quad  d = (d_c + d_s)$$
The task is to robustly predict the label $y_i$ from the given input data $x_i$. Note that we assume that the $\sigma^2_{\mathrm{spur}} \leq \sigma^2_{\mathrm{core}}$. This assumption, combined with the high correlation of the attribute $a$ with the label $y$, makes it easier for a learned linear model to rely on $x_{\mathrm{spur}}$ as predictive of $y$ over $x_{c_1}$ since the spurious-core information ratio $\sigma^2_{\mathrm{core}}/\sigma^2_{\mathrm{spur}}$ is high \citep{sagawa2020investigation}.
\subsection{Transfer Task : Prediction from noised input}
The transfer task is defined by $\mathbf{T}_{\mathrm{trans}} = \{(\tilde{x}_i, y^{\mathrm{trans}}_i)\}_{i \in M}$ where we have $M$ total samples. Figure \ref{img:aux_task_img} gives a visual depiction of how input samples for this task are constructed.  $M$ unlabelled points (with respect to the primary task) are taken from the distribution described by Equation \ref{eqn:prim_gen_dist}. Noise of the form :
\begin{equation}
\label{eqn:aux_gen_dist}
    \begin{split}
        % x_{\mathrm{spur}} ~|~ y &~ \sim \mathcal{N}\left(y\mathbf{1} ~,~ \sigma^2_{\mathrm{core}}I_{d^{t}_c} \right) \\
        x_{\mathrm{noise}} &~\sim \mathcal{N}\left(0 ~,~ \sigma^2_{\mathrm{noise}}I_{d^{t}_n} \right) \\
        d &= d^{t}_c+ d^{t}_n + d^{t}_s
    \end{split} 
\end{equation}
is applied to $d^{t}_n$ dimensions of the input.
Thus $d^{t}_c$, $d^{t}_s$ core and spurious feature dimensions respectively are left unnoised when compared to  Equation \ref{eqn:prim_gen_dist}. This generates $\tilde{x}_i$ from $x_i$. The transfer task is to predict the existence of some desired feature of the input. We thus assume that there exists some $w^{*}_{\mathrm{trans}}$ such that :
\begin{equation*}
    y_{\mathrm{trans}}  = \mathrm{sign}\left(\left(w^{*}_{\mathrm{trans}}\right)^T\tilde{x}\right)
\end{equation*}
$w^{*}_{\mathrm{trans}}$ is zero everywhere except in $d^{t}_c$ dimensions that correspond to the unnoised, original core feature dimensions.
To ground this in the birds example from Section \ref{sec:theory_motivation}, $\mathbf{T}_{\mathrm{trans}}$ can represent the task of predicting whether a noised image contains a beak. Whilst this task is not exactly self-supervised as motivated in Section \ref{sec:theory_motivation},  we contend that it is a reasonable proxy since it 1) shares core features with the end-task 2) leverages a large diverse pool of $M$ unlabelled (with respect to the end-task) data 3) is more amenable to theoretical analysis.

\subsection{Model}
\label{section:learning_model}
We multitask $\mathbf{T}_{\mathrm{trans}}$ with the end-task, $\mathbf{T}_{\mathrm{prim}}$. 
Modern multitask learning problems typically have a feature base $f(x)$ over model inputs that is jointly shared between tasks. Each task has a separate prediction head such that : 
$$y^{\mathrm{prim}}_{\mathrm{pred}} = \big(w^{\mathrm{prim}}\big)^Tf(x) \quad \text{and} \quad y^{\mathrm{trans}}_{\mathrm{pred}} = \big(w^{\mathrm{trans}}\big)^Tf(x)$$
For simplicity, the featurizer $f\left( \cdot \right)$ is a linear function $f : \mathbb{R}^{d} \rightarrow  \mathbb{R}^{d} ~|~ f_{\mathbf(a)}(x) = x^T\left(\mathrm{\textbf{diag}}(\mathbf{a})\right) $.

Let $\mathbf{A}\left(\tau \right) = \{\mathbf{a} \in R^{d} ~|~ \|\mathbf{a}\|_{1} \leq \tau \}$ be a set of $\ell_1$-norm constrained vectors and $\gamma > 0$ is a strictly positive margin. For a fixed weighting $\lambda > 0$, the joint multitask learning problem is as follows : 
\begin{equation}
    \begin{split}
        \mathbf{\Tilde{w}}^{\mathrm{trans}}, \mathbf{\Tilde{w}}^{\mathrm{prim}}, \mathbf{\Tilde{a}} ~=~ \mathrm{argmin}_{\|w^{\mathrm{trans}}\| =  \|w^{\mathrm{prim}}\| = 1, ~a ~\in~ \mathbf{A}\left(\tau \right)} \quad \lambda\mathcal{L_{\mathrm{t}}}\left(w^{\mathrm{trans}}, a \right) +  \mathcal{L_{\mathrm{p}}}\left(w^{\mathrm{prim}}, a \right)
    \end{split}
\end{equation}
\begin{equation*}
    \begin{split}
        \mathcal{L_{\mathrm{t}}}\left(w^{\mathrm{trans}}, a \right) &= \frac{1}{M}\sum_{(\tilde{x}_i, y^{\mathrm{trans}}_i) \in \mathbf{T}_{\mathrm{trans}}} \mathbf{1}\left[y^{\mathrm{trans}}_i\left(w^{\mathrm{trans}}\right)^Tf_{a}(\tilde{x}_i) \leq \gamma \right]\\ 
        \mathcal{L_{\mathrm{p}}}\left(w^{\mathrm{prim}}, a \right) &= \frac{1}{N}\sum_{(x_i, y_i) \in \mathbf{T}_{\mathrm{prim}}} \mathbf{1}\left[y_i\left(w^{\mathrm{prim}}\right)^Tf_{a}(x_i) \leq \gamma \right] 
    \end{split}
\end{equation*}

\subsection{Statement of Core Results}
\ld{Repeat the statement of core results here}


\section{Proof of core result}
\subsection{We can solve Equation \ref{Eqn:joint_eq}}
We can solve Equation \ref{Eqn:joint_eq} using Projected Gradient Descent since the set $\mathbf{A}\left(\tau \right)$ is convex. $w^{\mathrm{prim}}$ and $w^{\mathrm{trans}}$ can be normalized to unit norm after training.

\subsection{Lower bound on weight placed on core features for transfer-task}
We define the solution to the optimization problem defined by Equation \ref{Eqn:joint_eq} for the transfer task as :
$$\widetilde{w}^{\ast, \mathrm{trans}} = w^{\ast, \mathrm{trans}} \odot \mathbf{a}^\ast$$
Where $\odot$ is the Hadamard product. Let $y_{\mathrm{trans}}$ be the true label for the transfer task. The following statement on the population-error on the transfer task holds : 
\begin{equation}
    \label{eqn:upper_bound_test_err}
    \begin{split}
        \varepsilon^{\mathrm{trans}}_{\mathrm{test}} &= P\left(y_{\mathrm{trans}}\left(x\right)^{T}\widetilde{w}^{\ast, \mathrm{trans}} \leq \gamma\right) = P\left( \overline{\gamma}\left(x, y_{\mathrm{trans}}, \widetilde{w}^{\ast, \mathrm{trans}}\right) \leq \gamma \right) \\
        &= \sum_{(y_\mathrm{trans}, y, a) \in (\pm1, \pm1, \pm1)} w_{(y_\mathrm{trans}, y, a)}P\left( \overline{\gamma}\left(x, y_{\mathrm{trans}}, \widetilde{w}^{\ast, \mathrm{trans}}\right) \leq \gamma ~|~ y_{\mathrm{trans}}, y, a \right) \\
        &\geq \mathrm{min}_{(y_\mathrm{trans}, y, a) \in (\pm1, \pm1, \pm1)} ~ P\left( \overline{\gamma}\left(x, y_{\mathrm{trans}}, \widetilde{w}^{\ast, \mathrm{trans}}\right) \leq \gamma ~|~ y_{\mathrm{trans}}, y, a \right)  \\
         &\geq \mathrm{min}_{(y_\mathrm{trans}, y, a) \in (\pm1, \pm1, \pm1)} \quad \varepsilon^{y_{\mathrm{trans}}, y, a}_{\mathrm{test}} \\
    \end{split}
\end{equation}
We now characterize the distribution of $\overline{\gamma}\left(x, y_{\mathrm{trans}}, \widetilde{w}^{\ast, \mathrm{trans}}\right)$ for the case where  the result of the maximum in Equation \ref{eqn:upper_bound_test_err} is $P\left( \overline{\gamma}\left(x, y_{\mathrm{trans}}, \widetilde{w}^{\ast, \mathrm{trans}}\right) \leq \gamma ~|~ y_{\mathrm{trans}}= y = a = 1\right)$.  Note that the other seven terms gives the same bound when analyzed. \\
So, WLOG, we assume that $\varepsilon^{\mathrm{trans}, y_{\mathrm{trans}} = y = a = 1}_{\mathrm{test}} \leq \varepsilon^{\mathrm{trans}}_{\mathrm{test}}$
\begin{equation*}
    \begin{split}
        \overline{\gamma}\left(x, y_{\mathrm{trans}}, \widetilde{w}^{\ast, \mathrm{trans}}\right) &= \left(y_{\mathrm{trans}}(x_{\mathrm{core}})^T\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\right) + \left(y_{\mathrm{trans}}(x_{\mathrm{noise}})^T\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{noise}}\right) + \left(y_{\mathrm{trans}}(x_{\mathrm{spur}})^T\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\right) \\
        &= \mathcal{N}\left(~\left(\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\right)^T\mathbf{1}_{d^t_c} ~,~ \left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\| \sigma_{\mathrm{core}}\right)^2\right) + \mathcal{N}\left(0 ~,~ \left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{noise}}\| \sigma_{\mathrm{noise}}\right)^2\right) +  \\
        & + \mathcal{N}\left(~\left(\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\right)^T\mathbf{1}_{d^t_s} ~,~ \left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\| \sigma_{\mathrm{spur}}\right)^2\right) \\
        &= \mathcal{N}\left(\left(\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\right)^T\mathbf{1}_{d^t_c} + \left(\widetilde{w}^{\ast,\mathrm{trans}}_{\mathrm{spur}}\right)^T\mathbf{1}_{d^t_s} ~,~ \bigg(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|^2 \sigma_{\mathrm{core}}^2 + \|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{noise}}\|^2 \sigma_{\mathrm{noise}}^2 + \|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\|^2\sigma_{\mathrm{spur}}^2 \bigg) \right) \\
        &= \mathcal{N}\left(\overline{\mu}~,~ \overline{\sigma}^2 \right) \\
    \end{split}
\end{equation*}
Where
\begin{equation}
    \begin{split}
    \label{upper_bound_mean}
        \overline{\mu} &= \left(\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\right)^T\mathbf{1} + \left(\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\right)^T\mathbf{1} \\
        &\leq \sum_{i \in[d^t_c]} |\widetilde{w}^{\ast, \mathrm{trans}}_{i}| + \sum_{j \in[d^t_s]} |\widetilde{w}^{\ast, \mathrm{trans}}_{j}| \\
        &\leq  \bigg( \sum_{i \in[d^t_c]} |\mathbf{a}^{*, \mathrm{trans}}_{i}| \bigg)\bigg( \sum_{i \in [d^t_c]} |w^{\ast, \mathrm{trans}}_{i}| \bigg) + \bigg( \sum_{j \in[d^t_s]} |\mathbf{a}^{*, \mathrm{trans}}_{j}| \bigg)\bigg( \sum_{j \in[d^t_s]} |w^{\ast, \mathrm{trans}}_{j}| \bigg) \\
        &\leq d^t_c \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} + d^t_s \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\|_{1} \quad  \text{since} \quad \|w^{\ast, \mathrm{trans}}\|^2 = 1  \implies  \|w^{\ast, \mathrm{trans}}\|_{\infty} < 1\\
        &= (d^t_c - d^t_s) \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} + d^t_s \bigg( \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\|_{1} + \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} \bigg) \\
        &\leq (d^t_c - d^t_s) \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} + d^t_s \tau
    \end{split}
\end{equation}

and 
\begin{equation}
    \begin{split}
    \label{lower_bound_sigma}
        \overline{\sigma}^2 &= \left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\| \sigma_{\mathrm{core}}\right)^2 + \left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{noise}}\| \sigma_{\mathrm{noise}}\right)^2 + \left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\| \sigma_{\mathrm{spur}}\right)^2 \\
        \overline{\sigma}^2 &\geq \left( \sigma_{\mathrm{spur}}\right)^2\left(\|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|^2 + \|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{noise}}\|^2 + \|\widetilde{w}^{\ast, \mathrm{trans}}_{\mathrm{spur}}\|^2 \right)  \quad \text{since} \quad \sigma_{\mathrm{spur}} < \{\sigma_{\mathrm{core}}, \sigma_{\mathrm{noise}}\}\\
        &= \left(\sigma_{\mathrm{spur}}\right)^2\|\widetilde{w}^{\ast, \mathrm{trans}}\|^2 \\
        &\geq \left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}} \quad \text{From \ref{app_subsec:lowerbound_wtrans} we have that }
        \quad \|\widetilde{w}^{\ast, \mathrm{trans}}\|^2 \geq \eta^2_{\mathrm{trans}}
    \end{split}
\end{equation}

Let $z \sim \mathcal{N}\left(0, 1\right)$ be the standard normal distribution, then we have that : $\overline{\gamma} = \overline{\sigma}z + \overline{\mu}$
\begin{equation}
    \begin{split}
\label{eqn:core_features_lowerbound}
        \varepsilon^{\mathrm{trans}, (y = a)}_{\mathrm{test}} &=  P\left( \overline{\gamma} \leq \gamma \right) \\
        &= P\left(\overline{\sigma}z + \overline{\mu} \leq \gamma \right) \\ 
        &= P\left( z  \leq \frac{\gamma - \overline{\mu}}{\overline{\sigma}} \right) \\
        \Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y = a)}_{\mathrm{test}}\right) &= \frac{\gamma - \overline{\mu}}{\overline{\sigma}} \quad ~ \text{where} \quad \Phi^{-1} ~ \text{is the inverse Gaussian CDF}\\
        \overline{\sigma}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans, (y = a)}}_{\mathrm{test}}\right)\right) - \gamma &= \overline{\mu} \\
\overline{\sigma}^2\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y = a)}_{\mathrm{test}}\right)\right)^2 + \gamma^2 - 2\gamma\overline{\sigma}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y = a)}_{\mathrm{test}}\right)\right) &=  \overline{\mu}^2 
\end{split}
\end{equation}
We know that the margin $\gamma > 0$ and $\overline{\sigma} > 0$. We assume that we achieve better than random generalization error on test for the target task. This is a reasonable assumption to make with enough samples of the transfer task for training. Taking these together, we have that  $$\varepsilon^{\mathrm{trans}}_{\mathrm{test}} < 0.5 \implies \varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}} < 0.5 \implies \Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right) < 0 \implies -2\gamma\overline{\sigma}\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right) > 0$$
Thus, we have : 
\begin{equation}
\label{upper_bound_core_in_trans}
    \begin{split}
    \overline{\sigma}^2\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right)\right)^2 + \gamma^2 &\leq  \overline{\mu}^2 \\
\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}, (y=a)}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}}\right)\right)^2 + \gamma^2 &\leq  \overline{\mu}^2 \quad \text{from Equation \ref{lower_bound_sigma}}\\
\overline{\sigma}^2\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right)\right)^2 + \gamma^2 &\leq  \overline{\mu}^2 \\
\left(\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right)\right)^2 + \gamma^2 \right)^{\frac{1}{2}} &\leq \overline{\mu} \\
\left(\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right)\right)^2 + \gamma^2 \right)^{\frac{1}{2}} &\leq (d^t_c - d^t_s) \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} + d^t_s \tau \quad  \text{from Equation \ref{upper_bound_mean}} \\
\frac{1}{(d^t_c - d^t_s)}\bigg(\left(\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right)\right)^2 + \gamma^2 \right)^{\frac{1}{2}} - d^t_s\tau \bigg) &\leq \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} \\
\frac{1}{(d^t_c - d^t_s)}\bigg(\left(\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}}\right)\right)^2 + \gamma^2 \right)^{\frac{1}{2}} - d^t_s\tau \bigg) &\leq \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} \\
    \end{split}
\end{equation}
The last line for the result above is because :
\begin{equation*}
    \begin{split}
        \varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}} &\leq  \varepsilon^{\mathrm{trans}}_{\mathrm{test}} < 0.5  \\
        \implies \Phi^{-1}\left(\varepsilon^{\mathrm{trans}, (y=a)}_{\mathrm{test}}\right) &\leq \Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}}\right) < 0 \\
        \implies \left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}}\right)\right)^2 &\leq \left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}, (y=a)}\right)\right)^2  \\ 
    \end{split}
\end{equation*}
The result above is non-vacuous if the regularization is strong enough ie $\tau$ is small.
Now note that since $d^t_{c} \subset d_{c}$, we can apply the bound from Equation \ref{upper_bound_core_in_trans} to uppper bound $\|\mathbf{a}^{\ast, \mathrm{prim}}_{\mathrm{spur}}\|_{1}$
\begin{equation}
    \begin{split}
        \tau - \|\mathbf{a}^{\ast, \mathrm{prim}}_{\mathrm{spur}}\|_{1} = \|\mathbf{a}^{\ast, \mathrm{prim}}_{\mathrm{core}}\|_{1} &\geq \|\mathbf{a}^{\ast, \mathrm{trans}}_{\mathrm{core}}\|_{1} \geq \frac{1}{(d^t_c - d^t_s)}\bigg(\left(\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}}\right)\right)^2 + \gamma^2 \right)^{\frac{1}{2}} - d^t_s\tau \bigg) \\
        \|\mathbf{a}^{\ast, \mathrm{prim}}_{\mathrm{spur}}\|_{1} &\leq \frac{1}{(d^t_c -d^t_s)}\bigg(\left(d^t_c - 2d^t_s\right)\tau - \left(\left(\sigma_{\mathrm{spur}}\right)^2\eta^2_{\mathrm{trans}}\left(\Phi^{-1}\left(\varepsilon^{\mathrm{trans}}_{\mathrm{test}}\right)\right)^2 + \gamma^2 \right)^{\frac{1}{2}} \bigg) \\
        &= \lambda \\
    \end{split}
\end{equation}

\section{Upper bounding the worst-group error for the target task}
We define the solution to the optimization problem defined by Equation \ref{Eqn:joint_eq} for the primary task as :
$$\widetilde{w}^{\ast} = w^{\ast} \odot \mathbf{a}^\ast$$
WLOG, let us consider the minority group where $\{y = 1 ~,~ a = -1\}$. The error on this group for the target task is : 
$$\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}} = P\left(y\left(x\right)^{T}\widetilde{w}^{\ast} \leq \gamma\right) = P\left( \overline{\gamma}\left(x_{\{y=-a=1\}}, ~y=1, ~\widetilde{w}^{\ast}\right) \leq \gamma \right)$$
We now characterize the distribution of $\overline{\gamma}\left(x_{\{y=-a=1\}}, ~y=1, ~\widetilde{w}^{\ast}\right)$
\begin{equation*}
    \begin{split}
        \overline{\gamma}\left(x_{\{y=-a=1\}}, ~y=1, ~\widetilde{w}^{\ast}\right) &= \left(y(x_{\mathrm{core}})^T\widetilde{w}^{\ast}_{\mathrm{core}}\right) + \left(y(x_{\mathrm{noise}})^T\widetilde{w}^{\ast}_{\mathrm{sp}}\right) \\
        &= \mathcal{N}\left(~\left(\widetilde{w}^{\ast}_{\mathrm{core}}\right)^T\mathbf{1} ~,~ \left(\|\widetilde{w}^{\ast}_{\mathrm{core}}\| \sigma_{\mathrm{core}}\right)^2\right) + \mathcal{N}\left(-\left(\widetilde{w}^{\ast}_{\mathrm{sp}}\right)^T\mathbf{1}  ~,~ \left(\|\widetilde{w}^{\ast}_{\mathrm{sp}}\| \sigma_{\mathrm{sp}}\right)^2\right) \\
        &= \mathcal{N}\left(\left(\widetilde{w}^{\ast}_{\mathrm{core}}\right)^T\mathbf{1} - \left(\widetilde{w}^{\ast}_{\mathrm{sp}}\right)^T\mathbf{1} ~,~ \left(\|\widetilde{w}^{\ast}_{\mathrm{core}}\| \sigma_{\mathrm{core}}\right)^2 + \left(\|\widetilde{w}^{\ast}_{\mathrm{sp}}\| \sigma_{\mathrm{sp}}\right)^2 \right) \\
        &= \mathcal{N}\left(\overline{\mu}~,~ \overline{\sigma}^2 \right) \\
    \end{split}
\end{equation*}
Where 
$$\overline{\mu} = \bigg( \left(\widetilde{w}^{\ast}_{\mathrm{core}}\right)^T\mathbf{1} - \left(\widetilde{w}^{\ast}_{\mathrm{sp}}\right)^T\mathbf{1}\bigg) = \overline{\mu}_{\mathrm{core}} - \overline{\mu}_{\mathrm{sp}}$$ 
and 
$$\overline{\sigma}^2 =\left(\|\widetilde{w}^{\ast}_{\mathrm{core}}\| \sigma_{\mathrm{core}}\right)^2 + \left(\|\widetilde{w}^{\ast}_{\mathrm{sp}}\| \sigma_{\mathrm{sp}}\right)^2$$
Let $z \sim \mathcal{N}\left(0, 1\right)$ be the standard normal distribution, then we have that : $\overline{\gamma} = \overline{\sigma}z + \overline{\mu}$
\begin{equation*}
    \begin{split}
        \varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}} &= P\left( \overline{\gamma} \leq \gamma \right) \\
        &= P\left(\overline{\sigma}z + \overline{\mu} \leq \gamma \right) \\ 
        &= P\left( z  \leq \frac{\gamma - \overline{\mu}}{\overline{\sigma}} \right) \\
        \Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right) &= \frac{\gamma - \overline{\mu}}{\overline{\sigma}} \\
        \overline{\sigma}^2\Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right)^2 \overline{\mu}^2  &= \gamma^2 \\
        &= \gamma^2 + (\overline{\mu}_{\mathrm{core}})^2 + (\overline{\mu}_{\mathrm{sp}})^2 - 2\overline{\mu}_{\mathrm{core}}\overline{\mu}_{\mathrm{sp}} + 2\gamma(\overline{\mu}_{\mathrm{sp}} - \overline{\mu}_{\mathrm{core}}) \\
        &= \gamma^2 + (\overline{\mu}_{\mathrm{core}})^2 + (\overline{\mu}_{\mathrm{sp}})^2 - 2\overline{\mu}_{\mathrm{core}}\overline{\mu}_{\mathrm{sp}} + 2\gamma(\overline{\mu}_{\mathrm{sp}} - \overline{\mu}_{\mathrm{core}}) \\
    \end{split}
\end{equation*}
We proceed to bound $|\overline{\mu}_{\mathrm{core}}|$ 
\begin{equation*}
    \begin{split}
        |\overline{\mu}_{\mathrm{core}}| &= |\left(\widetilde{w}^{\ast}_{\mathrm{core}}\right)^T\mathbf{1}| \\
        &\leq d_{c}\|\mathbf{a}^{\ast}_{\mathrm{core}}\|_{1} \quad \text{Following similar reasoning as Equation \ref{upper_bound_mean}}\\ 
    \end{split}
\end{equation*}
The bound on $|\overline{\mu}_{\mathrm{sp}}|$ follows similarly. 
We plug this back into our relation for $\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}$
\begin{equation*}
    \begin{split}
        \overline{\sigma}^2\Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right)^2 &\leq \gamma^2 + (\overline{\mu}_{\mathrm{core}})^2 + (\overline{\mu}_{\mathrm{sp}})^2 + 2|\overline{\mu}_{\mathrm{core}}||\overline{\mu}_{\mathrm{sp}}| + 2\gamma(|\overline{\mu}_{\mathrm{sp}}| + |\overline{\mu}_{\mathrm{core}}|) \\
        &\leq \gamma^2 + d^2_{c}\|\mathbf{a}^{\ast}_{\mathrm{core}}\|^2_1 + d^2_{sp}\|\mathbf{a}^{\ast}_{\mathrm{sp}}\|^2_1 + 2d_{c}d_{s}\|\mathbf{a}^{\ast}_{\mathrm{core}}\|_1\|\mathbf{a}^{\ast}_{\mathrm{sp}}\|_1 + 2\gamma(d_{s}\|\mathbf{a}^{\ast}_{\mathrm{sp}}\|_1 + d_{c}\|\mathbf{a}^{\ast}_{\mathrm{core}}\|_1 ) \\
        &\leq  \gamma^2 + d^2_{c}\tau^2 + d^2_{sp}\lambda^2 + 2d_{c}d_{sp}\tau\lambda + 2\gamma(d_{s}\lambda + d_{c}\tau ) \quad \text{since }~ \|\mathbf{a}^{\ast}_{\mathrm{core}}\| \leq \tau ~\text{and}~ \|\mathbf{a}^{\ast}_{\mathrm{sp}}\| \leq \lambda \\
        &=  \gamma^2 + \left(d_{c}\tau + d_{s}\lambda\right)(d_{c}\tau + d_{sp}\lambda + 2\gamma)  \\
    \end{split}
\end{equation*}
We take a detour to lower-bound ~$\overline{\sigma}^2$
\begin{equation*}
    \begin{split}
        \overline{\sigma}^2 &= \left(\|\widetilde{w}^{\ast}_{\mathrm{core}}\| \sigma_{\mathrm{core}}\right)^2 + \left(\|\widetilde{w}^{\ast}_{\mathrm{sp}}\| \sigma_{\mathrm{sp}}\right)^2 \\
        &= \left(\sigma_{\mathrm{core}}^2 - \sigma_{\mathrm{sp}}^2\right)\|\widetilde{w}^{\ast}_{\mathrm{core}}\|^2 +  \sigma_{\mathrm{sp}}^2\left(\|\widetilde{w}^{\ast}_{\mathrm{core}}\|^2 + \|\widetilde{w}^{\ast}_{\mathrm{sp}}\|^2\right) \\
        &=  \left(\sigma_{\mathrm{core}}^2 - \sigma_{\mathrm{sp}}^2\right)\|\widetilde{w}^{\ast}_{\mathrm{core}}\|^2 + \sigma_{\mathrm{sp}}^2\|\widetilde{w}^{\ast}\|^2 \\
        &\geq \sigma_{\mathrm{sp}}^2\|\widetilde{w}^{\ast}\|^2 \quad \text{Since we take that }~ \sigma_{\mathrm{core}} > \sigma_{\mathrm{sp}} \\
        &\geq \sigma_{\mathrm{sp}}^2 \frac{\gamma^2}{\eta^2_{\mathrm{prim}}} \quad \text{From previous Section \ref{subsec:lower_bound_on_w_norm} where we have a lower bound on}~ \|\widetilde{w}^{\ast}\|^2\\ 
    \end{split}
\end{equation*}
We plug this lower bound back into the original equation : 
\begin{equation*}
    \begin{split}
\overline{\sigma}^2\Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right)^2 
        &\leq \gamma^2 + \left(d_{c}\tau + d_{sp}\lambda\right)(d_{c}\tau + d_{sp}\lambda + 2\gamma)\\ 
        \left(\sigma_{\mathrm{sp}}^2 \frac{\gamma^2}{\eta^2_{\mathrm{prim}}}\right)\Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right)^2 &\leq \overline{\sigma}^2\Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right) \leq \gamma^2 + \left(d_{c}\tau + d_{sp}\lambda\right)(d_{c}\tau + d_{sp}\lambda + 2\gamma)\\
        \Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right)^2 &\leq \bigg(\frac{\eta^2_{\mathrm{prim}}}{\gamma^2\sigma^2_{sp}}\bigg)\bigg(\gamma^2 + \left(d_{c}\tau + d_{sp}\lambda\right)(d_{c}\tau + d_{sp}\lambda + 2\gamma)\bigg) \\
        \Phi^{-1}\left(\varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}}\right) &\leq -\bigg(\frac{\eta_{\mathrm{prim}}}{\gamma\sigma_{sp}}\bigg)\sqrt{\bigg(\gamma^2 + \left(d_{c}\tau + d_{sp}\lambda\right)(d_{c}\tau + d_{sp}\lambda + 2\gamma)\bigg)} \\
        \varepsilon^{\mathrm{prim}}_{\mathrm{test}, \{y = -a = 1\}} &\leq \Phi\bigg(-\bigg(\frac{\eta_{\mathrm{prim}}}{\gamma\sigma_{sp}}\bigg)\sqrt{\bigg(\gamma^2 + \left(d_{c}\tau + d_{sp}\lambda\right)(d_{c}\tau + d_{sp}\lambda + 2\gamma)\bigg)} \bigg) \\
    \end{split}
\end{equation*}

\subsection{Lower bound on $\|\widetilde{w}^{\ast}\|^2$}
\label{subsec:lower_bound_on_w_norm}
We proceed to lower bound $\|\widetilde{w}^{\ast}\|^2$ with high probability. Note that if we achieve a training error on the primary task of $\varepsilon_{tr}$, then given that we have $N$ points in total, we, have that for $(1 - \varepsilon_{tr})N$ points : 
$$y_i\left(\widetilde{w}^{\ast}\right)x_i \geq \gamma \implies \gamma \leq \|\widetilde{w}^{\ast}\|\|x_i\|$$

We note that $x_{i, \mathrm{core}} \sim \mathcal{N}\left(y_i\mathbf{1}, \sigma^2_{\mathrm{core}}\mathbf{I}_{d_c}\right)$ and thus $z_i = \left(x_{i, \mathrm{core}} - y_i\mathbf{1}\right) \sim \mathcal{N}\left(0, \sigma^2_{\mathrm{core}}\mathbf{I}_{d_c}\right)$ 
\begin{equation*}
\begin{split}
        \|z_i\|^2 &= \|x_{i, \mathrm{core}} - y_i\mathbf{1}\|^2 \\
        &= \|x_{i, \mathrm{core}}\|^2  + \|y_i\mathbf{1}\|^2 - 2 \left(y_ix_{i, \mathrm{core}}\right)^T\mathbf{1} \\
        &= \|x_{i, \mathrm{core}}\|^2  + \left(d_c\right)^2 - 2 \left(x_{i, \mathrm{core}}\right)^T\mathbf{1} \\
        \text{Note that with} & \text{ high probability} \\
        (1 + c_1)\sigma_{\mathrm{core}}^2 &\geq \|z_i\|^2 \quad \text{Where $c_1$ is a function of $N$ and $\varepsilon_{tr}$} ~\implies  c_1 = c_1
        \bigg(N(1 - \varepsilon_{tr})\bigg)\\
        \text{and thus}& \\
        (1 + c_1)\sigma_{\mathrm{core}}^2 &\geq \|x_{i, \mathrm{core}}\|^2  + \left(d_c\right)^2 - 2 \left(x_{i, \mathrm{core}}\right)^T\mathbf{1} \\
         &\geq \|x_{i, \mathrm{core}}\|^2  + \left(d_c\right)^2 - \alpha\|x_{i, \mathrm{core}}\|^2 - \frac{\left(d_c\right)^2}{\alpha} \quad \text{CS and Young's inequality} ~~ 0 < \alpha < 1 \\
          &\geq \left(1 - \alpha\right) \|x_{i, \mathrm{core}}\|^2  +  \frac{\left(d_c\right)^2\left(\alpha - 1\right)}{\alpha} \\
        \alpha(1 - \alpha)\|x_{i, \mathrm{core}}\|^2 &\leq \alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_c\right)^2 \\
        \|x_{i, \mathrm{core}}\|^2 &\leq \frac{\alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_c\right)^2}{\alpha(1 - \alpha)} \\
\end{split}
\end{equation*}
The same steps can be followed to derive the following with high probability : 
$$ \|x_{i, \mathrm{sp}}\|^2 \leq \frac{\alpha(1 + c_2)\sigma_{\mathrm{sp}}^2 + \left(1 - \alpha\right)\left(d_{sp}\right)^2}{\alpha(1 - \alpha)}$$
So we have that : 
\begin{equation}
    \begin{split}
    \label{Eqn:upper_bound_norm_of_x}
        \|x_i\|^2 &= \|x_{i, \mathrm{sp}}\|^2 +  \|x_{i, \mathrm{core}}\|^2 \\
        &\leq \frac{\alpha(1 + c_2)\sigma_{\mathrm{sp}}^2 + \left(1 - \alpha\right)\left(d_{sp}\right)^2 + \alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_{c}\right)^2}{\alpha(1 - \alpha)}  \\
        \|x_i\| &\leq \eta_{\mathrm{prim}} \quad \text{Where }~ \eta_{\mathrm{prim}} = \left(\frac{\alpha(1 + c_2)\sigma_{\mathrm{sp}}^2 + \left(1 - \alpha\right)\left(d_{sp}\right)^2 + \alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_{c}\right)^2}{\alpha(1 - \alpha)}\right)^{\frac{1}{2}}\\
    \end{split}
\end{equation}

From Equation \ref{Eqn:upper_bound_norm_of_x}, we have that, with high probability: 
$$\gamma \leq \|\widetilde{w}^{\ast}\|\eta_{\mathrm{prim}} \implies \|\widetilde{w}^{\ast}\|^2 \geq \frac{\gamma^2}{\eta^2_{\mathrm{prim}}}$$

\subsection{Lower bound on $\|\widetilde{w}^{\ast, \mathrm{trans}}\|^2$}
\label{app_subsec:lowerbound_wtrans}
We follow exactly the same argument as Section \ref{subsec:lower_bound_on_w_norm} above to lower bound $\|\widetilde{w}^{\ast, \mathrm{trans}}\|^2$ with high probability. 

\ld{Uncomment out and fix the rest of below}

% Note that if we achieve a training error on the transfer task of $\varepsilon^{\mathrm{trans}}_{tr}$, then given that we have $M$ points in total, we, have that for $(1 - \varepsilon^{\mathrm{trans}}_{tr})M$ points : 
% $$y_i\left(\widetilde{w}^{\ast, \mathrm{trans}}\right)x_i \geq \gamma \implies \gamma \leq \|\widetilde{w}^{\ast, \mathrm{trans}}\|\|x_i\|$$

% We note that $x_{i, \mathrm{core}} \sim \mathcal{N}\left(y_i\mathbf{1}, \sigma^2_{\mathrm{core}}\mathbf{I}_{d_c}\right)$ and thus $z_i = \left(x_{i, \mathrm{core}} - y_i\mathbf{1}\right) \sim \mathcal{N}\left(0, \sigma^2_{\mathrm{core}}\mathbf{I}_{d^t_c}\right)$ 
% \begin{equation*}
% \begin{split}
%         \|z_i\|^2 &= \|x_{i, \mathrm{core}} - y_i\mathbf{1}\|^2 \\
%         &= \|x_{i, \mathrm{core}}\|^2  + \|y_i\mathbf{1}\|^2 - 2 \left(y_ix_{i, \mathrm{core}}\right)^T\mathbf{1} \\
%         &= \|x_{i, \mathrm{core}}\|^2  + \left(d_c\right)^2 - 2 \left(x_{i, \mathrm{core}}\right)^T\mathbf{1} \\
%         \text{Note that with} & \text{ high probability} \\
%         (1 + c_1)\sigma_{\mathrm{core}}^2 &\geq \|z_i\|^2 \quad \text{Where $c_1$ is a function of $N$ and $\varepsilon_{tr}$} ~\implies  c_1 = c_1
%         \bigg(N(1 - \varepsilon_{tr})\bigg)\\
%         \text{and thus}& \\
%         (1 + c_1)\sigma_{\mathrm{core}}^2 &\geq \|x_{i, \mathrm{core}}\|^2  + \left(d_c\right)^2 - 2 \left(x_{i, \mathrm{core}}\right)^T\mathbf{1} \\
%          &\geq \|x_{i, \mathrm{core}}\|^2  + \left(d_c\right)^2 - \alpha\|x_{i, \mathrm{core}}\|^2 - \frac{\left(d_c\right)^2}{\alpha} \quad \text{CS and Young's inequality} ~~ 0 < \alpha < 1 \\
%           &\geq \left(1 - \alpha\right) \|x_{i, \mathrm{core}}\|^2  +  \frac{\left(d_c\right)^2\left(\alpha - 1\right)}{\alpha} \\
%         \alpha(1 - \alpha)\|x_{i, \mathrm{core}}\|^2 &\leq \alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_c\right)^2 \\
%         \|x_{i, \mathrm{core}}\|^2 &\leq \frac{\alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_c\right)^2}{\alpha(1 - \alpha)} \\
% \end{split}
% \end{equation*}
% The same steps can be followed to derive the following with high probability : 
% $$ \|x_{i, \mathrm{sp}}\|^2 \leq \frac{\alpha(1 + c_2)\sigma_{\mathrm{sp}}^2 + \left(1 - \alpha\right)\left(d_{sp}\right)^2}{\alpha(1 - \alpha)}$$
% So we have that : 
% \begin{equation}
%     \begin{split}
%     \label{Eqn:upper_bound_norm_of_x}
%         \|x_i\|^2 &= \|x_{i, \mathrm{sp}}\|^2 +  \|x_{i, \mathrm{core}}\|^2 \\
%         &\leq \frac{\alpha(1 + c_2)\sigma_{\mathrm{sp}}^2 + \left(1 - \alpha\right)\left(d_{sp}\right)^2 + \alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_{c}\right)^2}{\alpha(1 - \alpha)}  \\
%         \|x_i\| &\leq \eta_{\mathrm{prim}} \quad \text{Where }~ \eta_{\mathrm{prim}} = \left(\frac{\alpha(1 + c_2)\sigma_{\mathrm{sp}}^2 + \left(1 - \alpha\right)\left(d_{sp}\right)^2 + \alpha(1 + c_1)\sigma_{\mathrm{core}}^2 + \left(1 - \alpha\right)\left(d_{c}\right)^2}{\alpha(1 - \alpha)}\right)^{\frac{1}{2}}\\
%     \end{split}
% \end{equation}

% From Equation \ref{Eqn:upper_bound_norm_of_x}, we have that, with high probability: 
% $$\gamma \leq \|\widetilde{w}^{\ast}\|\eta_{\mathrm{prim}} \implies \|\widetilde{w}^{\ast}\|^2 \geq \frac{\gamma^2}{\eta^2_{\mathrm{prim}}}$$


==> unused_sections/introduction_ssl_neurips.tex <==
\section{Introduction}
\ak{SSL@NeurIPS Intro} \\
% \gncomment{Right now it's not very clear if this is a methods paper or an examination paper? Is the main point that you're proposing a useful method or providing an interesting insight? You should probably choose one and lean into that.}
Multi-tasking \citep{caruana1997multitask, baxter2000model, ruder2019transfer} with self-supervised learning based auxiliary objectives (MTL-SSL) has proven to be a powerful tool for improving a model's aggregate performance on a desired end-task \cite{dery2021should, dery2021auxiliary, loh2022surrogate}. Congruently, as learned systems exert ever-increasing influence on the real world, it is paramount that they not only perform well on aggregate but also exhibit equitable outcomes across diverse subgroups characterized by attributes such as race \citep{buolamwini2018gender, liang2021towards}, gender \citep{buolamwini2018gender, srinivasan2021worst}, and geographies \citep{de2019does, ayush2021geography}. However, despite the strides made from leveraging SSL via multi-task learning, and the widely acknowledged importance of equitable machine learning, previous work has neither examined the effect of MTL-SSL on worst-group outcomes nor sought to design effective strategies that leverage said approach to achieve more equitable outcomes. In this paper, we attempt to fill this gap.

Traditionally, the problem of poor group-based outcomes has been tackled \emph{explicitly} via methods such as distributionally robust optimization (DRO) \citep{ben2013robust, sagawa2019distributionally, pmlr-v139-zhou21g, setlur2023bitrate}. In DRO, instead of finding parameters $\theta$ that minimize the expected risk $\ell$ over the training distribution (i.e. empirical risk minimization - ERM), the worst-case risk over a pre-defined set of distributions (the \emph{uncertainty set}) is instead minimized. 
% \gncomment{The rest of this paragraph isn't really true. There are lots of methods that do not require group annotations, e.g.~\citep{pmlr-v139-liu21f,michel2021modeling,oren-etal-2019-distributionally}. It should be rephrased.}
Since designing an appropriate uncertainty set generally requires \emph{explicit} access to group annotations at training time (which are unavailable in many practical settings),   several works have been proposed to tackle the challenges of worst-group generalization with little to no access to group annotations. These efforts often fall into two categories. The first category consists of methods that employ a two-stage training framework where examples with high loss are identified in the first stage and a second re-training stage appropriately refocuses on these examples \cite{NEURIPS2020_eddc3427, pmlr-v139-liu21f, pmlr-v162-zhang22z, nam2022spread, pmlr-v202-qiu23c, izmailov2022feature}. By virtual of requiring two passes over the data, these methods tend to increase training overhead. On the other hand, the second category involves unsupervised discovery of latent groups \cite{NEURIPS2020_e0688d13, paranjape2023agro} which can increase complexity at training time and thus deterring their wide usage. 
In contrast, this paper empirically demonstrates that  MTL-SSL can \emph{implicitly} improve the worst-group performance without incuring the overhead of two-stage training, costly acquisition of group labels, or the instantiation of complex models.

In general, poor group outcomes occur when a model relies on spurious features (the ones irrelevant to the task's group-based test accuracy) instead of core features (those necessary to robustly solve the task) during training. A carefully chosen auxiliary task would be one that, when multi-tasked with the end-task, encourages a model to use core features as opposed to spurious ones. In this paper, we explore self-supervised learning tasks as candidates for multi-tasking.
Our choice of MTL-SSL as an intervention for worst-case group performance is inspired by previous work like \cite{hendrycks2019using} that show that transfer learning can improve model robustness. 
Moreover, given the widespread adoption of SSL objectives in both pre-training and multi-tasking to enhance average-case performance, it prompts the question of how this approach affects worst-case group performance. Taken these together, it is reasonable to anticipate that a thoughtfully designed variant of MTL-SSL will similarly enhance worst-case accuracy. Note that the MTL-SSL as a counter-measure alone may not be effective if the model has enough capacity to use the spurious features for the end-task and the core features for the self-supervised task. We therefore augment MTL-SSL framework with $\ell_1$ regularization on the model's final layer activation order to restrict capacity right before end-task prediction. Regularization causes the SSL task to act as a constraint, forcing the model (due to limited capacity) to ignore spurious features whilst focusing on core features in order to do well on both tasks.

We empirically validate our MTL-SSL intervention against worst-case group performance across experiments in natural language processing (NLP) and computer vision (CV). Through a battery of experiments, we demonstrate that MTL using the self-supervision based pre-training objective with $\ell_1$ regularization on a pre-trained model's final layer activations is competitive when pitted against state-of-the-art DRO approaches like JTT (Just-Train-Twice) \citep{pmlr-v139-liu21f} and BR-DRO (Bitrate-Constrained DRO) \citep{setlur2023bitrate}. In settings where validation group annotations are available, across $3$ widely used datasets, we outperform JTT and BR-DRO on $3$ and $2$ tasks, respectively using our regularized MTL approach with end-task data only. Our approach improves worst-case group accuracy over ERM (by as much as $\sim 4\%$) and JTT (by $\sim 1\%$) in settings where group annotations are completely unavailable. We ablate our method across a wide range of settings: varying the choice of SSL auxiliary task, using only end-task data versus external data, and training with a pre-trained model versus training a model from scratch. Our results demonstrate that multi-tasking the end-task with a self-supervised learning objective  can be a versatile and robust tool against poor group-based outcomes.
